Hamiltonian Dynamics Learning from Point Cloud Observations for Nonholonomic Mobile Robot Control

Reliable autonomous navigation requires adapting the control policy of a mobile robot in response to dynamics changes in different operational conditions. Hand-designed dynamics models may struggle to capture model variations due to a limited set of parameters. Data-driven dynamics learning approaches offer higher model capacity and better generalization but require large amounts of state-labeled data. This paper develops an approach for learning robot dynamics directly from point-cloud observations, removing the need and associated errors of state estimation, while embedding Hamiltonian structure in the dynamics model to improve data efficiency. We design an observation-space loss that relates motion prediction from the dynamics model with motion prediction from point-cloud registration to train a Hamiltonian neural ordinary differential equation. The learned Hamiltonian model enables the design of an energy-shaping model-based tracking controller for rigid-body robots. We demonstrate dynamics learning and tracking control on a real nonholonomic wheeled robot.

==> tex/todo.tex <==
% \section{TODO}
% {\color{blue} 
% \begin{itemize}
%     \item Define $SO(3)$ and $SE(3)$ spaces and their tangent spaces along with the maps
%     \item Comparison with a baseline kinematic-based control law, e.g, “Closed loop steering of unicycle like vehicles via Lyapunov techniques”
%     \item Experiments: (1) Maneuvering through obstacles to show the advantage of learning the dynamics (2) Tire inflation and added payload (3) Moving on an inclined/declined plane? 
    
% \end{itemize}

% }
